Parallel MMF: a Multiresolution Approach to Matrix Computation

Multiresolution Matrix Factorization (MMF) was recently introduced as a method for finding multiscale structure and defining wavelets on graphs/matrices. In this paper we derive pMMF, a parallel algorithm for computing the MMF factorization. Empirically, the running time of pMMF scales linearly in the dimension for sparse matrices. We argue that this makes pMMF a valuable new computational primitive in its own right, and present experiments on using pMMF for two distinct purposes: compressing matrices and preconditioning large sparse linear systems.

==> experiments.tex <==
\section{Experiments}\label{sec: experiments}

\input{implementation}


==> implementation.tex <==
\section{Implementation}\label{sec: implementation}

We implemented pMMF in C++11 with the goal of building a general purpose library that scales to large matrices. 
Critical to the implementation are the data structures used to store blocked vectors and matrices, which must support 
\setlength{\plitemsep}{0pt}
\begin{inparaenum}[(a)]%[1.]
\item Sparsity,
\item Block level parallelism,
\item Fast multiplication by Givens rotations and \m{k}--point rotations from both the left and the right,  
\item Fast computation of inner products between columns (and of Gram matrices),  
\item Fast reblocking, 
\item Fast matrix/vector multiplication. 
\end{inparaenum} 
Since we could not find any existing matrix libary fulfilling all these requirements, we implemented the 
blocked matrix data structure from scratch directly on top of the \texttt{stl::vector},  
\texttt{stl::list} and \texttt{stl::hash\_map} containers. 
The source code of the project will be made publicly available under the GNU Public License \cite{gpl}. 

The main parameters of pMMF are the order of the rotations, \m{k}, 
the number of stages, \m{P}, the target number of clusters per stage, \m{m}, and the 
compression ratio, \m{\eta}, which is the number of rotations to perform in a given 
cluster, as a function of the cluster size. In most of our experiments, 
a single row/column is removed from the active set 
after each rotation. For computational efficiency, we use a rough randomized clustering 
method, which selects \m{m} ``anchors columns'' uniformly at random from the active set, 
and clusters the remaining columns to the anchor column with which is has highest normalized 
inner product. The clustering method has additional parameters intended to ensure the clustering 
is approximately even. 
If the size of any of the clusters falls below \m{c_{\text{min}}}, then 
its columns are redistributed amongst the remaining clusters, whereas if the size of any of the clusters 
exceeds \m{c_{\text{max}}}, then its columns are recursively reclustered using the same algorithm. 
The maximum recursion depth is \m{D_{\text{max}}}. There is also a bypass flag, which, when set, 
signifies that rows/columns which could not be successfuly clustered using the above method at 
a given stage will simply bypass the stage, with no rotations applied to them. 
Setting these parameters on a given system requires some experience, 
but overall our results appear stable w.r.t. the parameter values (including \m{p}, \m{m} and \m{\eta)}, 
as long as they are in a reasonable range. 


